Maximal Dissent: a State-Dependent Way to Agree in Distributed Convex Optimization

Consider a set of agents collaboratively solving a distributed convex optimization problem, asynchronously, under stringent communication constraints. In such situations, when an agent is activated and is allowed to communicate with only one of its neighbors, we would like to pick the one holding the most informative local estimate. We propose new algorithms where the agents with maximal dissent average their estimates, leading to an information mixing mechanism that often displays faster convergence to an optimal solution compared to randomized gossip. The core idea is that when two neighboring agents whose distance between local estimates is the largest among all neighboring agents in the network average their states, it leads to the largest possible immediate reduction of the quadratic Lyapunov function used to establish convergence to the set of optimal solutions. As a broader contribution, we prove the convergence of max-dissent subgradient methods using a unified framework that can be used for other state-dependent distributed optimization algorithms. Our proof technique bypasses the need of establishing the information flow between any two agents within a time interval of uniform length by intelligently studying convergence properties of the Lyapunov function used in our analysis.

==> local-global.tex <==

\subsection{Local Max-Gossip}\label{sec:LMG}

The standard gossiping algorithm described above is state-independent in the sense that the selection of the \textit{gossiping edge} $e$ does not depend on the states at the agents at any time. One pertinent question is: 
-- If an agent $i$, upon being randomly selected, could chose one of its neighbors to gossip based on the value of their state, which one should it be?  The answer is that with maximal dissent.

\um{Thus, we consider the neighbor selection strategy which
gossips} with the neighbor $j\in \mathcal{N}_{i}$ that has the largest\footnote{In case there are multiple solutions to \cref{eq:max}, we may select the agent with the smallest index, without loss of optimality.} possible state discrepancy (maximal dissent) with $i$, i.e.,
\begin{equation}\label{eq:max}
    j = \arg \max_{j\in \mathcal{N}_{i}} \|\vecx_j(t) - \vecx_{i}(t) \|.
\end{equation}
The selection rule in \cref{eq:max} was  introduced in~\cite{ustebay2010greedy} under the moniker \textit{Greedy Gossip with Eavesdropping}. Herein, we refer to this scheme as \textit{Local Max-Gossip}. The main intuition is very simple: with the goal of accelerating the convergence to the average of the initial states in the presence of the information regarding the neighbors' current state, gossiping with a neighbor with the largest disagreement leads to the largest possible immediate reduction in the Lyapunov function used to capture the variance of the states in the network. 

Since the edge over which the gossiping occurs depends on the current state of the neighbors, the resulting averaging matrix is a state-dependent, random matrix. For a sequence of independently and uniformly distributed index sequence $\{s(t)\}$, the Local Max-Gossip dynamics can be written as a state-dependent averaging scheme as follows %\eqref{eq:stateconsensus} 
\begin{equation}\label{eq:localmaxmat}
    A\big(t,X(t)\big)=\Agossip\Big(\big\{s(t),r_{s(t)}\big(X(t)\big)\big\}\Big),
\end{equation}
where 
\begin{equation}\label{eqn:rsxt}
    % r_s(X) = \arg \max_{r:\{s,r\}\in\Ecal}\|\vecx_s-\vecx_r\| 
    r_s(X) = \arg \max_{r\in \Ncal_s}\|\vecx_s-\vecx_r\|.
\end{equation}
%is  a neighbor with the maximum disagreement from $s$ for a given state matrix $X$. 

%Note that in the event that $\Scal_s\triangleq \argmax_{r\in\Ncal_s}\{\vecx_s - \vecx_r\}$ has more than one element $r_s(X)$ is chosen uniformly at random from $\Scal_s.$


%Mathematically, \textit{local max-gossip} the averaging matrix $A(t)=A(X(t))$ is a matrix defined through the process of gossip-based averaging over the \textit{locally} most ``different'' edges amongst a nodes' connections, on the network. 

%Mathematically, for a network $\Gcal=(\Vcal,\Ecal)$, given a node $s \in \Vcal$, and a matrix $X \in \R^{n\times d}$( representing the state of the agents), we define a local max-edge $e_s(X) \triangleq \{s,r_s(X)\},$ 

%Also, let us define the gossiping matrix over an edge $e=\{i,j\}\in \Ecal$ by 
%\begin{align}
%\Agossip(e)\triangleq I - \frac{1}{2}(\vec{b}_{i}-\vec{b}_{j})(\vec{b}_{i}-\vec{b}_{j})^T. \label{eq:matrix_form_1}
%\end{align}

%Then, the proposed max-gossip subgradient method adopts the dynamics 
%\begin{align}
%    W(t+1) &= A(\e(X(t))X(t), \label{eq:maxgossip_do1} \\\nonumber  
%    X(t+1) &= W(t+1) - \alpha(t+1)G(t+1), %\label{eq:maxgossip_do2}
%\end{align}
%where $\alpha(t+1) = \frac{1}{t+1}$, and $\vec{g}_i(t+1)\in \partial f_i(w_i(t+1))$ for all $i\in[n]$ and $t\geq 0$. 

\begin{remark}
The authors of~\cite{ustebay2010greedy} have also proved that the Local Max-Gossip averaging scheme converges faster than the standard randomized gossip algorithm. However, the characterization of the convergence rate is, essentially, an intractable problem. This is due to the intricate inter-temporal dependence of the state-dependent gossiping matrices. Nevertheless, empirical evidence clearly shows that Local Max-Gossip, when available, results in a significant gain over state-independent gossiping with respect to convergence rates.
\end{remark}



%\todo[inline]{B: please complete this.}

%Now we define $\Agossip(\elmg(X))$ as a gossiping matrix determined by the edge $\elmg(X) \triangleq \{s,r_s(X)\}$ which is a random variable. Here, 
%the node $s$ of the edge is chosen uniformly at random from the set of agents in $\Vcal$ and the other node of the edge is chosen to be the `furthest' node with respect to the node values amongst the neighbors of $s$ that can be defined as a function of $s$ and $X$ as follow:
% \begin{align}
%     r_s{(X)} \in \arg\max_{r \in \Ncal_{s}} \|\vecx_s - \vecx_r\|.
% \end{align}
% %for all $t\geq 0$.
% The averaging scheme defined through local max-gossip above is a generalization of the consensus scheme discussed as Greedy Gossip with Eavesdropper in~\cite{ustebay2010greedy} for vector-valued nodes. 
%Following the above definition we can also define $\node_s(w(t))$ where the other node is chosen to be furthest from node $s$ with respect to $w(t)$ instead of $x(t)$, that is,
%\begin{align}
%    \node_s(\vec{w}(t)) \triangleq \arg\max_{r \in \Ncal_{s}} |w_s(t) - w_r(t)|.
%\end{align}

%%Satisfying convergent property
%\begin{lemma}\label{lemma:lmgContraction}
%Averaging matrix in local max-gossip protocol, $\Almg \triangleq A(\elmg(X))$, satisfies Assumption \ref{asmpn:quadraticprop}, i.e., 
%\begin{align}
%    \E[V(\Almg(X)X)] \leq \lambda V(X),
%\end{align}
%where $\lambda \in (0,1)$ and the expectation is with respect to the distribution of $\Almg$.
%\end{lemma}

\subsection{Global Max-Gossip}

%% From local max-gossip to a better option, descriptive intro to algo
%% mathematical description
%% Lack of decentralization
%%

Local Max-Gossip can be further improved by choosing the edge connecting the agents with the largest possible disagreement among all edges in the graph $\Gcal = (\Vcal, \Ecal)$, i.e.,
\begin{equation}
    \emax(\Gcal, X) =  \arg \max_{\{i,j\}\in\Ecal}\|\vecx_i-\vecx_j\|. \label{eq:emax}
\end{equation}
In case there are multiple solutions to \cref{eq:emax}, we select the smallest pair of indices $(i^*,j^*)$ based on the lexicographical order, without loss of optimality. For brevity, we use $\emax(X)$ to denote the \textit{max-edge}. 
%for any discussion when the graph is static. 

%We will include $\Gcal_t$ in the notation for any discussion regarding time-varying communication graphs.   

%In the case there are multiple edges in the set of solutions to \eqref{eq:emax}, any choice (deterministic or random) of elements in $\emax(X)$ would be an equally valid choice. 
%In local max-gossip algorithm, we are faithful to the general structure of the gossip algorithm: at each iteration a node is selected at random, and then it chooses the maximum different local neighbor to gossip with. 

\um{The resulting algorithm is termed \textit{Max-Gossip} and serves as a benchmark as to what is achievable via state-dependent averaging schemes.  Max-gossip requires an oracle to provide the edge resulting in the largest possible Lyapunov function reduction across all network edges.  A question for future work is to determine whether a decentralized method exists which offers performance between that of Max-Gossip and Local Max-Gossip.}
%The resulting algorithm is called \textit{Max-Gossip}, and can be interpreted as an if oracle that informs us about which edge to select such that leads to the largest possible immediate reduction in the Lyapunov function associated with the variance of the states across the \textit{entire} network. Clearly, Global-Max improves upon its local counterpart. However, it does not admit a direct decentralized implementation. Nevertheless, Max-Gossip serves as a benchmark as to what is achievable in terms of state-dependent averaging algorithms.  


%In this case, in fact, A sample path of the local max-gossip algorithm is a special case when the node selected at random belongs to the edge with the maximum disagreement over the network. 
%For such a sample path the locally most ``different" edge is also the {\em globally} most ``different" edge.
%Here, by an instance we refer to a realization of the random matrix $A(\elmg(X))$.  We refer to this special instance of local-max gossip averaging matrix as the global max-gossip averaging matrix. 
%Therefore, during every iteration the global max-gossip averaging algorithm essentially selects the edge over which the exchange taking place is the one with the most disagreement across the entire network. 

%Mathematically, for a network $\Gcal=(\Vcal,\Ecal)$ and state estimates $X\in \R^{n\times d}$, we define the max-edge $\emax(X)\in \Ecal$ to be an edge that carries the maximum ``distance" between two adjacent nodes in $\Gcal$, {\em i.e.}, 

Given an initial state matrix $X(0)$, the Max-Gossip averaging scheme admits a state-dependent dynamics of the form %\cref{eq:stateconsensus} as follows
\begin{equation}\label{eqn:maxgossip}
    A\big(t,X(t)\big) = B\Big(\emax\big(X(t)\big)\Big),
\end{equation}
where the gossiping matrix is given by \cref{eq:matrix_form_1} and the max-edge is selected according to \cref{eq:emax}. Using arguments similar to \cite[Theorem~2]{ustebay2010greedy}%\todo{B:which theorem?}
, it can be shown that the Max-Gossip has a faster convergence rate than the Local Max-Gossip algorithm. However, the complete characterization of its convergence rate also seems to be an intractable problem. 
 
 
%where $\emax(X(t)) \in \argmax_{\{i,j\}\in\Ecal}\|\vecx_i(t)-\vecx_j(t)\|$.
%Then, the proposed max-gossip subgradient method adopts the dynamics 
%\begin{align}
%    W(t+1) &= A(\emax(X(t))X(t), \label{eq:maxgossip_do1} \\\nonumber  
%    X(t+1) &= W(t+1) - \alpha(t+1)G(t+1), %\label{eq:maxgossip_do2}
%\end{align}
%where $\alpha(t+1) = \frac{1}{t+1}$, and $\vec{g}_i(t+1)\in \partial f_i(\vecw_i(t+1))$ for all $i\in[n]$ and $t\geq 0$. The main result of this work establishes the convergence guarantees for this dynamics as stated below. 
%\begin{lemma}\label{lemma:maxContraction}
%Averaging matrix in local max-gossip protocol, $\Amg \triangleq A(\emax(X))$, satisfies Assumption \ref{asmpn:quadraticprop}, that is, 
%\begin{align}
%    \E[V(\Amg(X)X)] \leq \lambda V(X),
%\end{align}
%where $\lambda \in (0,1)$.
%\end{lemma}



%Note that if, for the sample paths of the Local Max-Gossip scheme with gossiping matrices \cref{eq:localmaxmat},  %where
%the updating node $s(t)$ belongs to a max-edge for all $t$,  then the Local Max-Gossip scheme coincides with the Max-Gossip scheme. 




%For such a sample path the locally most ``different" edge is also the {\em globally} most ``different" edge.
%Here, by an instance we refer to a realization of the random matrix $A(\elmg(X))$.  We refer to this special instance of local-max gossip averaging matrix as the global max-gossip averaging matrix. 
%Therefore, during every iteration the global max-gossip averaging algorithm essentially selects the edge over which the exchange taking place is the one with the most disagreement across the entire network. 

%This global max-gossip averaging scheme converges faster than local max-gossip algorithm.


